Teacher Perception of Automatically Extracted Grammar Concepts for L2 Language Learning

One of the challenges in language teaching is how best to organize rules regarding syntax, semantics, or phonology in a meaningful manner. This not only requires content creators to have pedagogical skills, but also have that language's deep understanding. While comprehensive materials to develop such curricula are available in English and some broadly spoken languages, for many other languages, teachers need to manually create them in response to their students' needs. This is challenging because i) it requires that such experts be accessible and have the necessary resources, and ii) describing all the intricacies of a language is time-consuming and prone to omission. In this work, we aim to facilitate this process by automatically discovering and visualizing grammar descriptions. We extract descriptions from a natural text corpus that answer questions about morphosyntax (learning of word order, agreement, case marking, or word formation) and semantics (learning of vocabulary). We apply this method for teaching two Indian languages, Kannada and Marathi, which, unlike English, do not have well-developed resources for second language learning. To assess the perceived utility of the extracted material, we enlist the help of language educators from schools in North America to perform a manual evaluation, who find the materials have potential to be used for their lesson preparation and learner evaluation.

==> background.tex <==
\section{Background}
% describe what is Autolex and related work , its motivation, the pipeline, main findings from the paper. and here what you use it for

As mentioned above, popular NLP tasks of POS tagging \cite{toutanvoa-manning-2000-enriching} and dependency parsing \cite{kiperwasser-goldberg-2016-simple} provide  answers to questions such as ``what is the function  of a word'' or ``what are the syntactic relations between words''.
Over the past decade, these technologies have seen a revolution due to the application of ``deep learning'' \cite{goldberg2017neural}, which can automatically discover patterns in underlying data and have led to notable accuracy gains  for many tasks (e.g. POS tagging \cite{state}, syntactic \cite{kulmizev-etal-2019-deep}, and morphological analysis \cite{kondratyuk-straka-2019-75}).
Although the amount of in-language annotated data required to create effective systems is falling rapidly \cite{goldwater-griffiths-2007-fully,agic-etal-2015-bit}, large-scale databases of syntactically annotated data such as the Universal Dependencies (UD) treebanks \cite{nivre-etal-2006-talbanken05,nivre2016universal} have made reasonably sized data available in a variety of languages, 
and have set the stage for the use of syntactic analyses for diverse languages.

While the above-cited works mainly focus on local analysis of individual examples, these analyses can also form the basis for answering more global questions about the grammar.
For example, a linguist interested in understanding the typical word order (e.g.~subject-verb-object) may perform dependency parsing to identify verbs, subjects, and objects, and aggregate statistics about their relative order.
Prior work \cite{ostling-2015-word,wang-eisner-2017-fine} has looked at such analyses, but does not explain the conditions which trigger one order over the other.
\newcite{chaudhary-etal-2020-automatic} and \texttt{AutoLEX} \newcite{chaudhary2022autolex} have focused on extracting human- and machine-readable grammar patterns to describe morphological agreement, word order, and case marking processes, which were evaluated based on their intrinsic properties.
Specifically, we follow the  four steps defined by \texttt{AutoLEX} to extract the descriptions. 

\texttt{AutoLEX} takes as input a raw text corpus, comprising of sentences in the language of interest, and produces human- and machine-readable explanations of different linguistic behaviors.
The first step is formulating a linguistic question into an NLP task. 
For example, given a question ``how are objects ordered with respect to verbs in English'', they formalize it into the following NLP task ``predict whether the object comes before or after the verb''.
The second step is to learn a model for this prediction task, for which they construct the training data by identifying and extracting features from the text corpora that are known to govern the said phenomenon (e.g. POS tagging and dependency parsing to identify syntactic heads, subjects, verbs, etc.).
Next, they learn an algorithm, which allows them to extract not only the common patterns (e.g.~``object is before/after the verb'') but also the conditions which trigger each of them (e.g.~``objects come after verbs except for interrogatives'').
Importantly, for each pattern, illustrative examples with examples of exceptions are extracted from the corpora.
Finally, they visualize the extracted conditions with illustartive examples through an online interface.
This process is illustrated in Figure \ref{fig:autolex}.
In this paper, we take a step further by examining the utility of such extracted descriptions for second language education of Marathi and Kannada.



==> images/autolex-usability-results-marathi.tex <==
\begin{table*}[t]
%\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|l|l|l}
    %\toprule
    \textbf{Grammar Concept} & \textbf{Relevance} & \multicolumn{2}{c|}{\textbf{Utility}} & \textbf{Presentation}  \\
    & \textbf{\% of relevant} & \textbf{\% of teachers} & \textbf{\% of teachers } & \textbf{\% of teachers} \\
    & \textbf{curriculum covered} & \textbf{likely to use} & \textbf{that would use for} & \textbf{found this \rule{1cm}{0.15mm} to navigate} \\
    \toprule 
    General Information & 15\% & highly likely: - & \textbf{lesson prep: 100\%} & very easy: - \\
                        &     & likely: 40\% & student exploration: 50\% &  \textbf{somewhat easy: 80\%} \\
                        & & \textbf{not likely: 60\%} & student evaluation: - &  difficult: 20\% \\
    \midrule
    Vocabulary & 16\% & highly likely: - & \textbf{lesson prep: 100\%} & 
    very easy: - \\
               &      & likely: 40\% & student exploration: 50\% & \textbf{somewhat easy: 100\%} \\
               & & \textbf{not likely: 60\%} & student evaluation: 50\% & difficult: - \\
    \midrule
    Suffix Usage & 9\% & highly likely: - & \textbf{lesson prep: 100\%} & very easy: - \\
     &     & likely: 40\% & student exploration: 50\% &  \textbf{somewhat easy: 100\%} \\
     & & \textbf{not likely: 60\%} & student evaluation: - & difficult: - \\
    \midrule
    Word Order & 8\% & highly likely: - & \textbf{lesson prep: 100\%} & very easy: - \\
     &     & likely: 40\% & student exploration: 50\% &  \textbf{somewhat easy: 80\%} \\
     & & \textbf{not likely: 60\%} & student evaluation: - & difficult: 20\% \\
    \midrule
    Agreement & 5\% & highly likely: - & \textbf{lesson prep: 100\%} & very easy: - \\
     &     & likely: 40\% & student exploration: 50\% &  \textbf{somewhat easy: 80\%} \\ 
     & & \textbf{not likely: 60\%} & student evaluation: - & difficult: 20\% \\
    \end{tabular}
    }
    \caption{Perception study results for Marathi. 5 teachers participated in this study}
    \label{tab:questionnaireresultsmarathi}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}

==> images/quality-study-questions.tex <==
\begin{table*}[t]
\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l}
    %\toprule
    Question & Answer Choices \\
    \midrule 
    1. Are the rules along with the accompanying examples  &
    a. precisely defining a linguistic distinction \\
    demonstrating the language property correctly?& b. too specific \\
    & c. too general \\
    & d. not corresponding to a real distinction in the language \\
    & e. cannot decide as incorrectly parsed \\
    
    \midrule
   2. What language learning level covers or should cover it?  & e.g. Textbook-1 \\
              
    \midrule
   3.1 If this material has already been covered,  & Yes/No \\
        could you still use some of our material & \\
        to enrich your existing material? & \\
    \midrule
    3.2 If the material is not already covered,  & Yes/No \\
    would you add this in your teaching & \\

    \end{tabular}
    }
    \caption{Questions asked to the Kannada experts for evaluating the quality and overall fit of the material.}
    \label{tab:qualityquestions}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}

==> images/relatedwordsummary.tex <==
\begin{table*}[t]
\small
    %\vspace{-.1cm}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|c|c}
    \toprule
  Linguistic Phenomena &  Work & Rule-Type & Corpus Type   \\
    \midrule
  WordOrder & Ours & C+FG & Raw text\\
            & Grammar Matrix \cite{bender-etal-2002-grammar} & C+FG & IGT text* \\
            & \citet{lewis-xia-2008-automatically} & C &  IGT text \\
            & \citet{bender-etal-2013-towards} & C & IGT text \\
            & \citet{ostling-2015-word} & C & Raw text   \\
            & \citet{wang-eisner-2017-fine} & C & Raw text  \\
            & WALS \citet{wals} & C & Reference grammar* \\
  \midrule
  Case Marking & Ours & C+FG & Raw text \\
               & Grammar Matrix \cite{bender-etal-2002-grammar} & C+FG & IGT text* \\
               & WALS \citet{wals} & C & Reference grammar* \\
               & \citet{howell-etal-2017-inferring} & C & IGT text \\
    \midrule
    Agreement &  Ours & C+FG & Raw text \\
              & Grammar Matrix \cite{bender-etal-2002-grammar} & C+FG & IGT text* \\
              & \citet{chaudhary-etal-2020-automatic} & C+FG & Raw text \\
              
    \midrule 
    Sentence construction & \citet{hellan-2010-descriptive} & FG & IGT text* \\
   
    \end{tabular}
    }
    \caption{An overview of linguistic questions \emph{automatically} answered by our current work and existing related work. Some of them combine semi-automatic approaches with manually annotated resources, there are marked with *. Rule-Type  denotes the type of rule extracted for a language, C refers to coarse-grained  such as rules for canonical word order, FG refers to fine-grained i.e. rules extracted at a local level. 
    % \gn{I feel like it might be nicer if we had one column for each linguistic phenomenon like ``word order'', ``case marking'', ``morphological agreement'', ``morphological paradigms'' etc. And you could add a differernt symbol for ``canonical'' (``C''?) and fine-grained (``FG''?) in each column for each work that handles those things?} 
    }
    \label{tab:relatedwork}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}

==> images/systemoverview.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/Pipeline.pdf}
    \caption{An overview of the \textsc{AutoLEX} framework  (with Adj-N order in Spanish as an example). The example sentence translates to \emph{Four books were bought by the small girl}. First, we formulate a linguistic question (e.g.~regarding Adj-N order) as a binary classification task (e.g.~``whether the Adj comes before/after the N'). Next, we perform syntactic analysis on the raw text, from which we extract syntactic, lexical, and semantic features to construct the training data. Finally, we learn an interpretable model from which we  extract concise rules. 
    %\an{Might help if we number the steps of the process on the figure and also refer to these in the caption (and potentially in the main body text)?}
    %\aditi{added}
    }
    \label{fig:systemoverview}
    \vspace{-1em}
\end{figure*}

==> images/vocab-eval-example.tex <==
% district (NOUN)	"ಜಿಲ್ಲಾಡಳಿತ (jilladlit)
% ಜಿಲ್ಲಾ (jilla)
% ಜಿಲ್ಲಾಸ್ಪತ್ರೆ (jillaspatre)
% ಜಿಲ್ಲಾಧಿಕಾರಿ (jilladhikari)
% ತಾಲ್ಲೂಕು (talluku)"	20	"1 is district administration
% 2 is accurate
% 3 is district hospital
% 4 is district official
% 5 is taluk"

\begin{table*}[t]
\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c}
    %\toprule
    English Word & Kannada Words & Expert Comment \\
    \midrule 
    temple (NOUN) & devsthan & district administration \\
                    & devalayas & district \\
                    & degul &  district hospital \\
                    & mandir & district official \\
                    
                    
    \midrule
   


    \end{tabular}
    }
    \caption{Vocabulary evaluation by Kannada experts. The Kannada word is written in the roman script for easy readability.\aditi{ask Arun/Ashwin for corrrect romanization of these words} }
    \label{tab:lingquestions}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}
